On a Standard Method for Measuring the Natural Rate of Interest

I show that Holston, Laubach and Williams' (2017) implementation of Median Unbiased Estimation (MUE) cannot recover the signal-to-noise ratio of interest from their Stage 2 model. Moreover, their implementation of the structural break regressions which are used as an auxiliary model in MUE deviates from Stock and Watson's (1998) formulation. This leads to spuriously large estimates of the signal-to-noise parameter $\lambda _{z}$ and thereby an excessive downward trend in other factor $z_{t}$ and the natural rate. I provide a correction to the Stage 2 model specification and the implementation of the structural break regressions in MUE. This correction is quantitatively important. It results in substantially smaller point estimates of $\lambda _{z}$ which affects the severity of the downward trend in other factor $z_{t}$. For the US, the estimate of $\lambda _{z}$ shrinks from $0.040$ to $0.013$ and is statistically highly insignificant. For the Euro Area, the UK and Canada, the MUE point estimates of $\lambda _{z}$ are \emph{exactly} zero. Natural rate estimates from HLW's model using the correct Stage 2 MUE implementation are up to 100 basis points larger than originally computed.

==> _abstract.tex <==
%TCIDATA{Version=5.50.0.2953}
%TCIDATA{LaTeXparent=0,0,hlw.2d.tex}


%%%%
%%%%
%%%%\documentclass[a4paper,final,12pt]{article}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%\usepackage[detect-all]{siunitx}
%%%%\usepackage{LaTexFiguresTablesStyle}
%%%%\usepackage[center,footnotesize]{subfigure}
%%%%
%%%%%TCIDATA{OutputFilter=LATEX.DLL}
%%%%%TCIDATA{Version=5.50.0.2953}
%%%%%TCIDATA{<META NAME="SaveForMode" CONTENT="2">}
%%%%%TCIDATA{BibliographyScheme=Manual}
%%%%%TCIDATA{LastRevised=Friday, November 22, 2019 11:15:01}
%%%%%TCIDATA{<META NAME="GraphicsSave" CONTENT="32">}
%%%%%TCIDATA{CSTFile=40 LaTeX dark article1.cst}
%%%%
%%%%\input{tcilatex}
%%%%\begin{document}
%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% UNCOMMENT ALL FROM THE TOP %%%%%%%%%%%%%%%%%%%%%%%%%
%%%\setstretch{1.27}

\begin{center}
\hspace*{-6mm}\textbf{Abstract}
\end{center}

\vspace*{2mm}\setstretch{1.07}%
% This paper provides estimates of the natural rate of interest from
% \citeauthor*{holston.etal:2017}' (\citeyear{holston.etal:2017}) structural
% model which

I show that Holston, Laubach and Williams' (2017) implementation of Median
Unbiased Estimation (MUE) cannot recover the signal-to-noise ratio of
interest from their Stage 2 model. Moreover, their implementation of the
structural break regressions which are used as an auxiliary model in MUE
deviates from Stock and Watson's (1998) formulation. This leads to spuriously
large estimates of the signal-to-noise parameter $\lambda _{z}$ and thereby
an excessive downward trend in other factor $z_{t}$ and the natural rate. I
provide a correction to the Stage 2 model specification and the
implementation of the structural break regressions in MUE. This correction is
quantitatively important. It results in substantially smaller point estimates
of $\lambda _{z}$ which affects the severity of the downward trend in other
factor $z_{t}$. For the US, the estimate of $\lambda _{z}$ shrinks from
$0.040$ to $0.013$ and is statistically highly insignificant. For the Euro
Area, the UK and Canada, the MUE point estimates of $\lambda _{z}$ are
\emph{exactly} zero. Natural rate estimates from HLW's model using the
correct Stage 2 MUE implementation are up to 100 basis points larger than
originally computed.

%These results suggest that there is little evidence of
%%These results suggest that the effect of `\emph{other factor}' $z_{t}$ on
%%the natural rate is considerably smaller than originally estimated by
%%Holston \emph{et al.} (2017).

%%%This paper corrects the implementation of Median Unbiased Estimation (MUE) in
%%%Stage 2 of Holston, Laubach and Williams' (2017) framework to estimate the
%%%natural rate of interest and provides corresponding corrected estimates. The
%%%correction is quantitatively important. It yields substantially smaller point
%%%estimates of the signal-to-noise ratio parameter $\lambda _{z}$ which
%%%determines the size of the downward trend of `\emph{other factor}' $z_{t}$ in
%%%the natural rate.
%%%For US data, the point estimate of $\lambda _{z}$ shrinks from $0.040$ to $%
%%%0.013$ and is statistically highly insignificant. For data on the Euro Area,
%%%the UK and Canada, the $\lambda _{z}$ point estimates are exactly zero.
%%%Natural rate estimates from this model are up to 100 basis points larger than
%%%originally computed by Holston \emph{et al.} (2017).

% indicating that the natural rate is solely determined by trend growth in this model.
\setstretch{1.0}%
\keywrds{Natural rate of interest, Median Unbiased Estimation, Kalman
Filter, misspecified econometric models, correction to Stage 2 model.}%
\newline
\jelclss{C32, E43, E52, O40.}\newline

%%\end{document}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% HTML/WEB ABSTRACT
%This paper corrects the implementation of Median Unbiased Estimation (MUE) in
%Stage 2 of Holston, Laubach and Williams' (2017) framework to estimate the
%natural rate of interest and provides cor&shy;re&shy;spond&shy;ing
%cor&shy;rect&shy;ed estimates. The correction is
%quan&shy;ti&shy;ta&shy;tive&shy;ly im&shy;por&shy;tant. It yields
%sub&shy;stan&shy;tial&shy;ly smaller point estimates of the signal-to-noise
%ratio pa&shy;ram&shy;e&shy;ter \(\lambda _{z}\) which de&shy;ter&shy;mines
%the size of the downward trend of <i>'other factor'</i> \(z_{t}\) in the
%natural rate. For US data, the point estimate of \(\lambda _{z}\) shrinks
%from 0.040 to 0.013 and is statistically highly insignificant. For data on
%the Euro Area, the UK and Canada, the \(\lambda _{z}\) point estimates are
%exactly zero. Natural rate estimates from this model are up to 100 basis
%points larger than originally computed by Holston <i>et al.</i> (2017).



%%I show that Holston, Laubach and Williams' (2017) implementation of Median
%%Unbiased Estimation (MUE) cannot recover the signal-to-noise ratio of
%%interest from their Stage 2 model. Moreover, their implementation of the
%%structural break regressions which are used as an auxiliary model in MUE
%%deviates from Stock and Watson's (1998) formulation. This leads to spuriously
%%large estimates of the signal-to-noise parameter \(\lambda _{z}\) and thereby
%%an excessive downward trend in other factor \(z_{t}\) and the natural rate. I
%%provide a correction to the Stage 2 model specification and the
%%implementation of the structural break regressions in MUE. This correction is
%%quantitatively important. It results in substantially smaller point estimates
%%of \(\lambda _{z}\) which affects the severity of the downward trend in other
%%factor \(z_{t}\). For the US, the estimate of \(\lambda _{z}\) shrinks from
%%0.040 to 0.013 and is statistically highly insignificant. For the Euro Area,
%%the UK and Canada, the MUE point estimates of \(\lambda _{z}\) are
%%<i>exactly</i> zero. Natural rate estimates from HLW's model using the
%%correct Stage 2 MUE implementation are up to 100 basis points larger than
%%originally computed.


==> _figstabs.tex <==
%%%\documentclass[a4paper,12pt,table]{article}
%%%\usepackage{dbPaper2021}
%%%\usepackage[round]{natbib}
%%%\usepackage[inner]{showlabels}
%%%\renewcommand{\showlabelsetlabel}[1]
%%%{\begin{turn}{90}\color{red}\showlabelfont \large #1\end{turn}}
%%%\geometry{left=20mm,right=20mm,top=21mm,bottom=23mm}
%%%\graphicspath{{../graphics/}{graphics/}}
%%%\newcommand{\FigandTabspace}{-11mm}
%%%\setlength{\footskip}{30pt}
%%%\setlength{\parskip}{05pt}
%%%\newcommand{\spce}{1.234}
%%%\def\plots{1}
%%%\begin{document}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%  -----------  UNCOMMENT ALL PACKAGES ABOVE THIS LINE THE TOP --------------------  %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\tabularxcolumn#1{m{#1}}
\renewcommand{\lbfnt}{\fontsize{9pt}{0pt}\selectfont} % std.err.  font size in tables
\renewcommand{\sefnt}{\fontsize{8pt}{0pt}\selectfont} % std.err.  font size in tables
\renewcommand{\pvfnt}{\fontsize{5pt}{0pt}\selectfont} % p-value   font size in tables
\newcommand{\capfnt}{\fontsize{10.5pt}{13pt}\selectfont} % std.err.  font size in tables
\renewcommand{\captionfont}{\capfnt\sf} %\renewcommand{\captionfont}{\small\sf}%\renewcommand{\captionfont}{\footnotesize\sf}
%{text height}{text width}{evenmargin}{odd margin}{columnsep}{topmargin}{headheight}{headsep}{footskip}
\changepage{33mm}{10mm}{-5mm}{-5mm}{00mm}{-4mm}{-11mm}{0mm}{-5.6mm}        % for a4paper
%\changepage{32mm}{5mm}{-2.5mm}{-2.5mm}{00mm}{-13mm}{-0mm}{0mm}{-1.575mm}    % for letterpaper
\setcounter{table}{0} \setcounter{figure}{0}
\renewcommand{\thefigure}{\arabic{figure}}%
\renewcommand{\thetable}{\arabic{table}}  %
\sisetup{detect-all}
% ------------------------------------------------------------------------------------
%\pagestyle{empty}

\vspace*{\FigandTabspace}
\section*{{Figures and Tables}}
\phantomsection\addcontentsline{toc}{section}{Figures and Tables}
\vspace*{77mm}
% --------------------------------------------------------------------------------------

\begin{figure}[h!]
\centering
\includegraphics[width=1\textwidth,trim={0 0 0 0},clip]{rec_estimates_US}
\vspace{-5mm}
\caption{Recursive ML estimates of $\sigma_g$ and $\sigma_z$ from HLW's full
model in \ref{eq:hlw} using HLW's initial values for the state vector. These results are based on US data, using an expanding
window of data from 1987:Q2 to 2019:Q4. The data were downloaded
from FRED on the 28$^{th}$ May 2020.}
\label{fig:US_rec_sigma_g}
\end{figure}

\cleardoublepage\newpage % ----------------------------------------------------------------------------------------

\begin{figure}[p!]
\centering
\includegraphics[width=1\textwidth,trim={0 0 0 0},clip]{Ftau_sw_hlw_2}
\vspace{-5mm}
\caption{Sequence of $F(\tau)$ statistics from SW's and HLW's implementation of the
structural break dummy variable regressions described in \ref{eq:sw_break} and
\ref{eq:sw_break_false}, respectively.}
\label{fig:SW_Fstats}
\end{figure}

\cleardoublepage\newpage % ----------------------------------------------------------------------------------------

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%                                     US
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\BT[p!]
\caption{Stage 2 parameter estimates for the US}\centering\vspace*{-2mm}%
\renewcommand{\arraystretch}{1.1}\renewcommand\tabcolsep{7pt}%
\fontsize{11pt}{13pt}\selectfont%
\newcolumntype{N}{S[table-format = 5.8,round-precision = 8, table-space-text-post={(}]}
\newcolumntype{U}{S[table-format = 5.8,round-precision = 8, table-space-text-post={(}]}
\newcolumntype{L}{S[table-format = 4.8,round-precision = 8, table-space-text-post={(}]}
\begin{tabular*}{.93\columnwidth}{p{30mm}NNNN}
\topline
\hsp[5]$\boldsymbol{\theta }_{2}$
& {\hsp[5]HLW.R-File\hsp[-0.0]}
& {\hsp[6]HLW\big($\hat\sigma_g^{\mathrm{MLE}}$\big)}
& {\hsp[6]Correct\hsp[-0]}
& {\hsp[5]Correct $+\,a_0$\hsp[-0]}\\
\midrule
  \input{table.input/Table_S2a_US.tex} \\[-5mm] \cmidrule(ll){1-5}
  \input{table.input/Table_S2b_US.tex} \\[-5mm]
\bottomrule
\end{tabular*}%
\tabnotes[-2.5mm][.925\columnwidth][-1.0mm]{\input{table.input/_table1_notes.tex}}%
\label{tab:US_Stage2}%
\ET

\cleardoublepage\newpage % ----------------------------------------------------------------------------------------

\begin{figure}[p!]
\centering \vspace{-2mm}
\includegraphics[width=1\textwidth,trim={0 0 0 0},clip]{US_Fstat_MUE2_Q4-2019.pdf}
\vspace{-5mm}
\caption{Sequence of $F(\tau)$ statistics from HLW's (misspecified) Stage 2 model and the correct Stage 2 model
defined in the left and right columns blocks of \ref{eq:S2} for the US. The red (HLW) and blue (SW) lines show respectively the $F(\tau)$ statistics of
the two different implementations of the structural break regressions given in equations \ref{d_hlw} to
\ref{d_true0}.}
\label{fig:US_Fstat}
\end{figure}

\cleardoublepage\newpage % ----------------------------------------------------------------------------------------

\BST[p!] \caption{Stage 2 MUE results of $\lambda_z$ with corresponding
structural break test statistics for the US} %
\centering\vspace*{-2mm}\renewcommand{%
\arraystretch}{1.1}\renewcommand\tabcolsep{7pt} %
\fontsize{11pt}{13pt}\selectfont %
\newcolumntype{N}{S[table-format = 2.6,round-precision = 6]} %
\newcolumntype{K}{S[table-format = 2.4,round-precision = 4]} %
\newcolumntype{Q}{S[table-format = 2.6,round-precision = 6]} %
\begin{tabular*}{.97\columnwidth}{p{8mm}NNKNKp{0mm}NKNKNK}
\topline
\multirow{2}{*}{\hsp[2]$\lambda_{z}$}
&     \multicolumn{5}{c}{HLW's implementation of structural break regressions}
&&    \multicolumn{6}{c}{SW's implementation of structural break regressions} \\ \cmidrule(rr){2-6} \cmidrule(lr){8-13}

& {\hsp[1]HLW.R-File}
& {\hsp[2]HLW\big($\hat\sigma_g^{\mathrm{MLE}}$\big)} & {\hsp[0][90\% CI]\hsp[2]}
& {\hsp[5]Correct\hsp[3]} & {\hsp[0][90\% CI]\hsp[2]}
& {}
& {\hsp[5]HLW \hsp[3]} & {\hsp[0][90\% CI]\hsp[2]}
& {\hsp[1]HLW\big($\hat\sigma_g^{\mathrm{MLE}}$\big)\hsp[-1]} & {\hsp[0][90\% CI]\hsp[2]}
& {\hsp[.5]Correct\hsp[-1]} & {\hsp[1][90\% CI]\hsp[3]} \\ \midrule
  \input{table.input/Table_MUEa_US.tex} \\[-5mm] \midrule \multirow{1}{*}{} & \multicolumn{9}{r}{Corresponding structural break test statistics ($p-$values in parenthesis)} \\ \midrule
  \input{table.input/Table_MUEb_US.tex} \\[-5mm]
\bottomrule
\end{tabular*}
\tabnotes[-2.2mm][.965\columnwidth][-1.5mm]{\input{table.input/_table2_notes.tex}}%
\label{tab:US_Stage2_lambda_z}%
\EST

\cleardoublepage\newpage % ----------------------------------------------------------------------------------------

\BT[p!]
\caption{Stage 3 parameter estimates for the US}\centering\vspace*{-2mm}%
\renewcommand{\arraystretch}{1.1}\renewcommand\tabcolsep{7pt}%
\fontsize{11pt}{13pt}\selectfont%
\newcolumntype{N}{S[table-format = 7.8,round-precision = 8, table-space-text-post={(}]}
\newcolumntype{U}{S[table-format = 7.8,round-precision = 8, table-space-text-post={(}]}
\newcolumntype{L}{S[table-format = 7.8,round-precision = 8, table-space-text-post={(}]}
\begin{tabular*}{.93\columnwidth}{p{46mm}NNN}
\topline
\hsp[5]$\boldsymbol{\theta }_{3}$
& {\hsp[9]HLW.R-File}
& {\hsp[8]MLE\big($\sigma_g|\hat\lambda_z^{\mathrm{Correct}}$\big)}
& {\hsp[10]MLE\big($\sigma_g,\sigma_z$\big)}\\
\midrule
  \input{table.input/Table_S3a_US.tex} \\[-5mm] \cmidrule(ll){1-4}
  \input{table.input/Table_S3b_US.tex} \\[-5mm]
\bottomrule
\end{tabular*}%
\tabnotes[-2.2mm][.925\columnwidth][-1.0mm]{\input{table.input/_table3_notes.tex}}%
\label{tab:US_Stage3}%
\ET

\cleardoublepage\newpage % ----------------------------------------------------------------------------------------

\begin{figure}[p!]
\centering \vspace{-2mm}
\includegraphics[width=1\textwidth,trim={0 0 0 0},clip]{US_estimates_filtered_HLW_prior_Q4-2019.pdf}
\vspace{-5mm}
\caption{Filtered estimates of the natural rate $r^{\ast}_t$,
annualized trend growth $g_t$, other factor $z_t$, and the output gap
(cycle) variable $\tilde{y}_t$ for the US.}
\label{fig:US_KF}
\end{figure}
\cleardoublepage\newpage % ----------------------------------------------------------------------------------------
\begin{figure}[p!]
\centering \vspace{-2mm}
\includegraphics[width=1\textwidth,trim={0 0 0 0},clip]{US_estimates_smoothed_HLW_prior_Q4-2019.pdf}
\vspace{-5mm}
\caption{Smoothed estimates of the natural rate $r^{\ast}_t$,
annualized trend growth $g_t$, other factor $z_t$, and the output gap
(cycle) variable $\tilde{y}_t$ for the US.}
\label{fig:US_KS}
\end{figure}

\cleardoublepage\newpage % ----------------------------------------------------------------------------------------


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%                                     EA
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\BT[p!]
\caption{Stage 2 parameter estimates for the Euro Area}\centering\vspace*{-2mm}%
\renewcommand{\arraystretch}{1.1}\renewcommand\tabcolsep{7pt}%
\fontsize{11pt}{13pt}\selectfont%
\newcolumntype{N}{S[table-format = 5.8,round-precision = 8, table-space-text-post={(}]}
\newcolumntype{U}{S[table-format = 5.8,round-precision = 8, table-space-text-post={(}]}
\newcolumntype{L}{S[table-format = 4.8,round-precision = 8, table-space-text-post={(}]}
\begin{tabular*}{.93\columnwidth}{p{30mm}NNNN}
\topline
\hsp[5]$\boldsymbol{\theta }_{2}$
& {\hsp[5]HLW.R-File\hsp[-0.0]}
& {\hsp[6]HLW\big($\hat\sigma_g^{\mathrm{MLE}}$\big)}
& {\hsp[6]Correct\hsp[-0]}
& {\hsp[5]Correct $+\,a_0$\hsp[-0]}\\
\midrule
  \input{table.input/Table_S2a_EA.tex} \\[-5mm] \cmidrule(ll){1-5}
  \input{table.input/Table_S2b_EA.tex} \\[-5mm]
\bottomrule
\end{tabular*}%
\tabnotes[-2.5mm][.925\columnwidth][-1.0mm]{\input{table.input/_table1_notes.tex}}%
\label{tab:EA_Stage2}%
\ET

\cleardoublepage\newpage % ----------------------------------------------------------------------------------------

\begin{figure}[p!]
\centering \vspace{-2mm}
\includegraphics[width=1\textwidth,trim={0 0 0 0},clip]{EA_Fstat_MUE2_Q4-2019.pdf} \vspace{-5mm}
%\caption{Sequence of $F$ statistics from the correctly and incorrectly specified Stage 2 models for the Euro Area}
\caption{Sequence of $F(\tau)$ statistics from HLW's (misspecified) Stage 2 model and the correct Stage 2 model
defined in the left and right columns blocks of \ref{eq:S2} for the Euro Area. The red (HLW) and blue (SW) lines show respectively the $F(\tau)$ statistics of
the two different implementations of the structural break regressions given in equations \ref{d_hlw} to
\ref{d_true0}.}
\label{fig:EA_Fstat}
\end{figure}

\cleardoublepage\newpage % ----------------------------------------------------------------------------------------

\BST[p!] \caption{Stage 2 MUE results of $\lambda_z$ with corresponding
structural break test statistics for the Euro Area} %
\centering\vspace*{-2mm}\renewcommand{%
\arraystretch}{1.1}\renewcommand\tabcolsep{7pt} %
\fontsize{11pt}{13pt}\selectfont %
\newcolumntype{N}{S[table-format = 2.6,round-precision = 6]} %
\newcolumntype{K}{S[table-format = 2.4,round-precision = 4]} %
\newcolumntype{Q}{S[table-format = 2.6,round-precision = 6]} %
\begin{tabular*}{.97\columnwidth}{p{8mm}NNKNKp{0mm}NKNKNK}
\topline
\multirow{2}{*}{\hsp[2]$\lambda_{z}$}
&     \multicolumn{5}{c}{HLW's implementation of structural break regressions}
&&    \multicolumn{6}{c}{SW's implementation of structural break regressions} \\ \cmidrule(rr){2-6} \cmidrule(lr){8-13}

& {\hsp[1]HLW.R-File}
& {\hsp[2]HLW\big($\hat\sigma_g^{\mathrm{MLE}}$\big)} & {\hsp[0][90\% CI]\hsp[2]}
& {\hsp[5]Correct\hsp[3]} & {\hsp[0][90\% CI]\hsp[2]}
& {}
& {\hsp[5]HLW \hsp[3]} & {\hsp[0][90\% CI]\hsp[2]}
& {\hsp[1]HLW\big($\hat\sigma_g^{\mathrm{MLE}}$\big)\hsp[-1]} & {\hsp[0][90\% CI]\hsp[2]}
& {\hsp[.5]Correct\hsp[-1]} & {\hsp[1][90\% CI]\hsp[3]} \\ \midrule
  \input{table.input/Table_MUEa_EA.tex} \\[-5mm] \midrule \multirow{1}{*}{} & \multicolumn{9}{r}{Corresponding structural break test statistics ($p-$values in parenthesis)} \\ \midrule
  \input{table.input/Table_MUEb_EA.tex} \\[-5mm]
\bottomrule
\end{tabular*}
\tabnotes[-2.2mm][.965\columnwidth][-1.5mm]{\input{table.input/_table2_notes.tex}}%
\label{tab:EA_Stage2_lambda_z}%
\EST

\cleardoublepage\newpage % ----------------------------------------------------------------------------------------

\BT[p!]
\caption{Stage 3 parameter estimates for the Euro Area}\centering\vspace*{-2mm}%
\renewcommand{\arraystretch}{1.1}\renewcommand\tabcolsep{7pt}%
\fontsize{11pt}{13pt}\selectfont%
\newcolumntype{N}{S[table-format = 7.8,round-precision = 8, table-space-text-post={(}]}
\newcolumntype{U}{S[table-format = 7.8,round-precision = 8, table-space-text-post={(}]}
\newcolumntype{L}{S[table-format = 7.8,round-precision = 8, table-space-text-post={(}]}
\begin{tabular*}{.93\columnwidth}{p{46mm}NNN}
\topline
\hsp[5]$\boldsymbol{\theta }_{3}$
& {\hsp[9]HLW.R-File}
& {\hsp[8]MLE\big($\sigma_g|\hat\lambda_z^{\mathrm{Correct}}$\big)}
& {\hsp[10]MLE\big($\sigma_g,\sigma_z$\big)}\\
\midrule
  \input{table.input/Table_S3a_EA.tex} \\[-5mm] \cmidrule(ll){1-4}
  \input{table.input/Table_S3b_EA.tex} \\[-5mm]
\bottomrule
\end{tabular*}%
\tabnotes[-2.2mm][.925\columnwidth][-1.0mm]{\input{table.input/_table3_notes.tex}}%
\label{tab:EA_Stage3}%
\ET

\cleardoublepage\newpage % ----------------------------------------------------------------------------------------

\begin{figure}[p!]
\centering \vspace{-2mm}
\includegraphics[width=1\textwidth,trim={0 0 0 0},clip]{EA_estimates_filtered_HLW_prior_Q4-2019.pdf}
\vspace{-5mm}
\caption{Filtered estimates of the natural rate $r^{\ast}_t$,
annualized trend growth $g_t$, other factor $z_t$, and the output gap
(cycle) variable $\tilde{y}_t$ for the Euro Area}
\label{fig:EA_KF}
\end{figure}
\cleardoublepage\newpage % ----------------------------------------------------------------------------------------
\begin{figure}[p!]
\centering \vspace{-2mm}
\includegraphics[width=1\textwidth,trim={0 0 0 0},clip]{EA_estimates_smoothed_HLW_prior_Q4-2019.pdf}
\vspace{-5mm}
\caption{Smoothed estimates of the natural rate $r^{\ast}_t$,
annualized trend growth $g_t$, other factor $z_t$, and the output gap
(cycle) variable $\tilde{y}_t$ for the Euro Area}
\label{fig:EA_KS}
\end{figure}

\cleardoublepage\newpage % ----------------------------------------------------------------------------------------

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%                                     UK
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\BT[p!]
\caption{Stage 2 parameter estimates for the UK}\centering\vspace*{-2mm}%
\renewcommand{\arraystretch}{1.1}\renewcommand\tabcolsep{7pt}%
\fontsize{11pt}{13pt}\selectfont%
\newcolumntype{N}{S[table-format = 5.8,round-precision = 8, table-space-text-post={(}]}
\newcolumntype{U}{S[table-format = 5.8,round-precision = 8, table-space-text-post={(}]}
\newcolumntype{L}{S[table-format = 4.8,round-precision = 8, table-space-text-post={(}]}
\begin{tabular*}{.93\columnwidth}{p{30mm}NNNN}
\topline
\hsp[5]$\boldsymbol{\theta }_{2}$
& {\hsp[5]HLW.R-File\hsp[-0.0]}
& {\hsp[6]HLW\big($\hat\sigma_g^{\mathrm{MLE}}$\big)}
& {\hsp[6]Correct\hsp[-0]}
& {\hsp[5]Correct $+\,a_0$\hsp[-0]}\\
\midrule
  \input{table.input/Table_S2a_UK.tex} \\[-5mm] \cmidrule(ll){1-5}
  \input{table.input/Table_S2b_UK.tex} \\[-5mm]
\bottomrule
\end{tabular*}%
\tabnotes[-2.5mm][.925\columnwidth][-1.0mm]{\input{table.input/_table1_notes.tex}}%
\label{tab:UK_Stage2}%
\ET

\cleardoublepage\newpage % ----------------------------------------------------------------------------------------

\begin{figure}[p!]
\centering \vspace{-2mm}
\includegraphics[width=1\textwidth,trim={0 0 0 0},clip]{UK_Fstat_MUE2_Q4-2019.pdf}
\vspace{-5mm}
%\caption{Sequence of $F$ statistics from the correctly and incorrectly specified
%Stage 2 models for the UK}
\caption{Sequence of $F(\tau)$ statistics from HLW's (misspecified) Stage 2 model and the correct Stage 2 model
defined in the left and right columns blocks of \ref{eq:S2} for the UK. The red (HLW) and blue (SW) lines show respectively the $F(\tau)$ statistics of
the two different implementations of the structural break regressions given in equations \ref{d_hlw} to
\ref{d_true0}.}
\label{fig:UK_Fstat}
\end{figure}

\cleardoublepage\newpage % ----------------------------------------------------------------------------------------

\BST[p!] \caption{Stage 2 MUE results of $\lambda_z$ with corresponding
structural break test statistics for the UK} %
\centering\vspace*{-2mm}\renewcommand{%
\arraystretch}{1.1}\renewcommand\tabcolsep{7pt} %
\fontsize{11pt}{13pt}\selectfont %
\newcolumntype{N}{S[table-format = 2.6,round-precision = 6]} %
\newcolumntype{K}{S[table-format = 2.4,round-precision = 4]} %
\newcolumntype{Q}{S[table-format = 2.6,round-precision = 6]} %
\begin{tabular*}{.97\columnwidth}{p{8mm}NNKNKp{0mm}NKNKNK}
\topline
\multirow{2}{*}{\hsp[2]$\lambda_{z}$}
&     \multicolumn{5}{c}{HLW's implementation of structural break regressions}
&&    \multicolumn{6}{c}{SW's implementation of structural break regressions} \\ \cmidrule(rr){2-6} \cmidrule(lr){8-13}

& {\hsp[1]HLW.R-File}
& {\hsp[2]HLW\big($\hat\sigma_g^{\mathrm{MLE}}$\big)} & {\hsp[0][90\% CI]\hsp[2]}
& {\hsp[5]Correct\hsp[3]} & {\hsp[0][90\% CI]\hsp[2]}
& {}
& {\hsp[5]HLW \hsp[3]} & {\hsp[0][90\% CI]\hsp[2]}
& {\hsp[1]HLW\big($\hat\sigma_g^{\mathrm{MLE}}$\big)\hsp[-1]} & {\hsp[0][90\% CI]\hsp[2]}
& {\hsp[.5]Correct\hsp[-1]} & {\hsp[1][90\% CI]\hsp[3]} \\ \midrule
  \input{table.input/Table_MUEa_UK.tex} \\[-5mm] \midrule \multirow{1}{*}{} & \multicolumn{9}{r}{Corresponding structural break test statistics ($p-$values in parenthesis)} \\ \midrule
  \input{table.input/Table_MUEb_UK.tex} \\[-5mm]
\bottomrule
\end{tabular*}
\tabnotes[-2.2mm][.965\columnwidth][-1.5mm]{\input{table.input/_table2_notes.tex}}%
\label{tab:UK_Stage2_lambda_z}%
\EST

\cleardoublepage\newpage % ----------------------------------------------------------------------------------------

\BT[p!]
\caption{Stage 3 parameter estimates for the UK}\centering\vspace*{-2mm}%
\renewcommand{\arraystretch}{1.1}\renewcommand\tabcolsep{7pt}%
\fontsize{11pt}{13pt}\selectfont%
\newcolumntype{N}{S[table-format = 7.8,round-precision = 8, table-space-text-post={(}]}
\newcolumntype{U}{S[table-format = 7.8,round-precision = 8, table-space-text-post={(}]}
\newcolumntype{L}{S[table-format = 7.8,round-precision = 8, table-space-text-post={(}]}
\begin{tabular*}{.93\columnwidth}{p{46mm}NNN}
\topline
\hsp[5]$\boldsymbol{\theta }_{3}$
& {\hsp[9]HLW.R-File}
& {\hsp[8]MLE\big($\sigma_g|\hat\lambda_z^{\mathrm{Correct}}$\big)}
& {\hsp[10]MLE\big($\sigma_g,\sigma_z$\big)}\\
\midrule
  \input{table.input/Table_S3a_UK.tex} \\[-5mm] \cmidrule(ll){1-4}
  \input{table.input/Table_S3b_UK.tex} \\[-5mm]
\bottomrule
\end{tabular*}%
\tabnotes[-2.2mm][.925\columnwidth][-1.0mm]{\input{table.input/_table3_notes.tex}}%
\label{tab:UK_Stage3}%
\ET

\cleardoublepage\newpage % ----------------------------------------------------------------------------------------

\begin{figure}[p!]
\centering \vspace{-2mm}
\includegraphics[width=1\textwidth,trim={0 0 0 0},clip]{UK_estimates_filtered_HLW_prior_Q4-2019.pdf}
\vspace{-5mm}
\caption{Filtered estimates of the natural rate $r^{\ast}_t$,
annualized trend growth $g_t$, other factor $z_t$, and the output gap
(cycle) variable $\tilde{y}_t$ for the UK}
\label{fig:UK_KF}
\end{figure}

\cleardoublepage\newpage % ----------------------------------------------------------------------------------------
\begin{figure}[p!]
\centering \vspace{-2mm}
\includegraphics[width=1\textwidth,trim={0 0 0 0},clip]{UK_estimates_smoothed_HLW_prior_Q4-2019.pdf}
\vspace{-5mm}
\caption{Smoothed estimates of the natural rate $r^{\ast}_t$,
annualized trend growth $g_t$, other factor $z_t$, and the output gap
(cycle) variable $\tilde{y}_t$ for the UK}
\label{fig:UK_KS}
\end{figure}

\cleardoublepage\newpage % ----------------------------------------------------------------------------------------

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%                                     CA
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\BT[p!]
\caption{Stage 2 parameter estimates for Canada}\centering\vspace*{-2mm}%
\renewcommand{\arraystretch}{1.1}\renewcommand\tabcolsep{7pt}%
\fontsize{11pt}{13pt}\selectfont%
\newcolumntype{N}{S[table-format = 5.8,round-precision = 8, table-space-text-post={(}]}
\newcolumntype{U}{S[table-format = 5.8,round-precision = 8, table-space-text-post={(}]}
\newcolumntype{L}{S[table-format = 4.8,round-precision = 8, table-space-text-post={(}]}
\begin{tabular*}{.93\columnwidth}{p{30mm}NNNN}
\topline
\hsp[5]$\boldsymbol{\theta }_{2}$
& {\hsp[5]HLW.R-File\hsp[-0.0]}
& {\hsp[6]HLW\big($\hat\sigma_g^{\mathrm{MLE}}$\big)}
& {\hsp[6]Correct\hsp[-0]}
& {\hsp[5]Correct $+\,a_0$\hsp[-0]}\\
\midrule
  \input{table.input/Table_S2a_CA.tex} \\[-5mm] \cmidrule(ll){1-5}
  \input{table.input/Table_S2b_CA.tex} \\[-5mm]
\bottomrule
\end{tabular*}%
\tabnotes[-2.5mm][.925\columnwidth][-1.0mm]{\input{table.input/_table1_notes.tex}}%
\label{tab:CA_Stage2}%
\ET

\cleardoublepage\newpage % ----------------------------------------------------------------------------------------

\begin{figure}[p!]
\centering \vspace{-2mm}
\includegraphics[width=1\textwidth,trim={0 0 0 0},clip]{CA_Fstat_MUE2_Q4-2019.pdf}
\vspace{-5mm}
\caption{Sequence of $F(\tau)$ statistics from HLW's (misspecified) Stage 2 model and the correct Stage 2 model
defined in the left and right columns blocks of \ref{eq:S2} for Canada. The red (HLW) and blue (SW) lines show respectively the $F(\tau)$ statistics of
the two different implementations of the structural break regressions given in equations \ref{d_hlw} to
\ref{d_true0}.}
%\caption{Sequence of $F$ statistics from the correctly and incorrectly specified
%Stage 2 models for Canada}
\label{fig:CA_Fstat}
\end{figure}

\cleardoublepage\newpage % ----------------------------------------------------------------------------------------

\BST[p!] \caption{Stage 2 MUE results of $\lambda_z$ with corresponding
structural break test statistics for Canada} %
\centering\vspace*{-2mm}\renewcommand{%
\arraystretch}{1.1}\renewcommand\tabcolsep{7pt} %
\fontsize{11pt}{13pt}\selectfont %
\newcolumntype{N}{S[table-format = 2.6,round-precision = 6]} %
\newcolumntype{K}{S[table-format = 2.4,round-precision = 4]} %
\newcolumntype{Q}{S[table-format = 2.6,round-precision = 6]} %
\begin{tabular*}{.97\columnwidth}{p{8mm}NNKNKp{0mm}NKNKNK}
\topline
\multirow{2}{*}{\hsp[2]$\lambda_{z}$}
&     \multicolumn{5}{c}{HLW's implementation of structural break regressions}
&&    \multicolumn{6}{c}{SW's implementation of structural break regressions} \\ \cmidrule(rr){2-6} \cmidrule(lr){8-13}

& {\hsp[1]HLW.R-File}
& {\hsp[2]HLW\big($\hat\sigma_g^{\mathrm{MLE}}$\big)} & {\hsp[0][90\% CI]\hsp[2]}
& {\hsp[5]Correct\hsp[3]} & {\hsp[0][90\% CI]\hsp[2]}
& {}
& {\hsp[5]HLW \hsp[3]} & {\hsp[0][90\% CI]\hsp[2]}
& {\hsp[1]HLW\big($\hat\sigma_g^{\mathrm{MLE}}$\big)\hsp[-1]} & {\hsp[0][90\% CI]\hsp[2]}
& {\hsp[.5]Correct\hsp[-1]} & {\hsp[1][90\% CI]\hsp[3]} \\ \midrule
  \input{table.input/Table_MUEa_CA.tex} \\[-5mm] \midrule \multirow{1}{*}{} & \multicolumn{9}{r}{Corresponding structural break test statistics ($p-$values in parenthesis)} \\ \midrule
  \input{table.input/Table_MUEb_CA.tex} \\[-5mm]
\bottomrule
\end{tabular*}
\tabnotes[-2.2mm][.965\columnwidth][-1.5mm]{\input{table.input/_table2_notes.tex}}%
\label{tab:CA_Stage2_lambda_z}%
\EST

\cleardoublepage\newpage % ----------------------------------------------------------------------------------------

\BT[p!]
\caption{Stage 3 parameter estimates for Canada}\centering\vspace*{-2mm}%
\renewcommand{\arraystretch}{1.1}\renewcommand\tabcolsep{7pt}%
\fontsize{11pt}{13pt}\selectfont%
\newcolumntype{N}{S[table-format = 7.8,round-precision = 8, table-space-text-post={(}]}
\newcolumntype{U}{S[table-format = 7.8,round-precision = 8, table-space-text-post={(}]}
\newcolumntype{L}{S[table-format = 7.8,round-precision = 8, table-space-text-post={(}]}
\begin{tabular*}{.93\columnwidth}{p{46mm}NNN}
\topline
\hsp[5]$\boldsymbol{\theta }_{3}$
& {\hsp[9]HLW.R-File}
& {\hsp[8]MLE\big($\sigma_g|\hat\lambda_z^{\mathrm{Correct}}$\big)}
& {\hsp[10]MLE\big($\sigma_g,\sigma_z$\big)}\\
\midrule
  \input{table.input/Table_S3a_CA.tex} \\[-5mm] \cmidrule(ll){1-4}
  \input{table.input/Table_S3b_CA.tex} \\[-5mm]
\bottomrule
\end{tabular*}%
\tabnotes[-2.2mm][.925\columnwidth][-1.0mm]{\input{table.input/_table3_notes.tex}}%
\label{tab:CA_Stage3}%
\ET

\cleardoublepage\newpage % ----------------------------------------------------------------------------------------

\begin{figure}[p!]
\centering \vspace{-2mm}
\includegraphics[width=1\textwidth,trim={0 0 0 0},clip]{CA_estimates_filtered_HLW_prior_Q4-2019.pdf}
\vspace{-5mm}
\caption{Filtered estimates of the natural rate $r^{\ast}_t$,
annualized trend growth $g_t$, other factor $z_t$, and the output gap
(cycle) variable $\tilde{y}_t$ for Canada}
\label{fig:CA_KF}
\end{figure}
\cleardoublepage\newpage % ----------------------------------------------------------------------------------------
\begin{figure}[p!]
\centering \vspace{-2mm}
\includegraphics[width=1\textwidth,trim={0 0 0 0},clip]{CA_estimates_smoothed_HLW_prior_Q4-2019.pdf}
\vspace{-5mm}
\caption{Smoothed estimates of the natural rate $r^{\ast}_t$,
annualized trend growth $g_t$, other factor $z_t$, and the output gap
(cycle) variable $\tilde{y}_t$ for Canada}
\label{fig:CA_KS}
\end{figure}

\cleardoublepage\newpage % ----------------------------------------------------------------------------------------





\newpage\cleardoublepage

%%\ifthenelse{\equal{1}{\plots}}{\end{document}}{}

\ifthenelse{\equal{1}{\plots}}{
\bibliographystyle{LongBibStyleFile}
\bibliography{DanielsBibTexLibrary}
\end{document}}{}


==> table.input/Table_MUEa_CA.tex <==
$L$ &  {\hsp[2]---} &  0.000000 &  {\hsp[-2][0, 0.01]} &  0.000000 &  {\hsp[-2][0, 0.01]} &   &  0.000000 &  {\hsp[-2][0, 0.01]} &  0.000000 &  {\hsp[-2][0, 0.01]} &  0.000000 &  {\hsp[-2][0, 0.01]} \\
MW  &  0.009032 		&  0.008855 &  {\hsp[-2][0, 0.06]} &  0.000000 &  {\hsp[-2][0, 0.01]} &   &  0.000000 &  {\hsp[-2][0, 0.01]} &  0.000000 &  {\hsp[-2][0, 0.01]} &  0.000000 &  {\hsp[-2][0, 0.02]} \\
EW  &  0.016314 		&  0.015288 &  {\hsp[-2][0, 0.07]} &  0.000000 &  {\hsp[-2][0, 0.01]} &   &  0.000000 &  {\hsp[-2][0, 0.01]} &  0.000000 &  {\hsp[-2][0, 0.01]} &  0.000000 &  {\hsp[-2][0, 0.02]} \\
QLR &  0.032111 		&  0.031447 &  {\hsp[-2][0, 0.11]} &  0.000000 &  {\hsp[-2][0, 0.01]} &   &  0.000000 &  {\hsp[-2][0, 0.02]} &  0.000000 &  {\hsp[-2][0, 0.02]} &  0.000000 &  {\hsp[-2][0, 0.03]} \\



==> table.input/Table_MUEa_EA.tex <==
$L$ &  {\hsp[2]---} &  0.000000 &  {\hsp[-2][0, 0.03]} &  0.000000 &  {\hsp[-2][0, 0.03]} &   &  0.000000 &  {\hsp[-2][0, 0.05]} &  0.000000 &  {\hsp[-2][0, 0.03]} &  0.000000 &  {\hsp[-2][0, 0.03]} \\
MW  &  0.024235 		&  0.021309 &  {\hsp[-2][0, 0.10]} &  0.000000 &  {\hsp[-2][0, 0.03]} &   &  0.000000 &  {\hsp[-2][0, 0.06]} &  0.000000 &  {\hsp[-2][0, 0.04]} &  0.000000 &  {\hsp[-2][0, 0.04]} \\
EW  &  0.032869 		&  0.025664 &  {\hsp[-2][0, 0.11]} &  0.000000 &  {\hsp[-2][0, 0.04]} &   &  0.005006 &  {\hsp[-2][0, 0.07]} &  0.000000 &  {\hsp[-2][0, 0.05]} &  0.000000 &  {\hsp[-2][0, 0.05]} \\
QLR &  0.044176 		&  0.040711 &  {\hsp[-2][0, 0.14]} &  0.000000 &  {\hsp[-2][0, 0.05]} &   &  0.020474 &  {\hsp[-2][0, 0.09]} &  0.006325 &  {\hsp[-2][0, 0.07]} &  0.001430 &  {\hsp[-2][0, 0.06]} \\

% {\hsp[2][0, 
% {\hsp[2][0, 
% {\hsp[2][0, 
% {\hsp[2][0, 

==> table.input/Table_MUEa_UK.tex <==
$L$ &  {\hsp[2]---} &  0.000000 &  {\hsp[-2][0, 0.03]} &  0.000000 &  {\hsp[-2][0, 0.03]} &   &  0.000000 &  {\hsp[-2][0, 0.03]} &  0.000000 &  {\hsp[-2][0, 0.03]} &  0.000000 &  {\hsp[-2][0, 0.03]} \\
MW  &  0.017600 		&  0.017855 &  {\hsp[-2][0, 0.08]} &  0.000000 &  {\hsp[-2][0, 0.02]} &   &  0.000000 &  {\hsp[-2][0, 0.04]} &  0.000000 &  {\hsp[-2][0, 0.04]} &  0.000000 &  {\hsp[-2][0, 0.04]} \\
EW  &  0.019307 		&  0.019860 &  {\hsp[-2][0, 0.08]} &  0.000000 &  {\hsp[-2][0, 0.03]} &   &  0.000000 &  {\hsp[-2][0, 0.05]} &  0.000000 &  {\hsp[-2][0, 0.05]} &  0.000000 &  {\hsp[-2][0, 0.05]} \\
QLR &  0.022484 		&  0.023628 &  {\hsp[-2][0, 0.09]} &  0.007219 &  {\hsp[-2][0, 0.05]} &   &  0.014437 &  {\hsp[-2][0, 0.07]} &  0.014828 &  {\hsp[-2][0, 0.07]} &  0.015647 &  {\hsp[-2][0, 0.07]} \\



==> table.input/Table_MUEa_US.tex <==
$L$ &  {\hsp[2]---} &  0.000000 &  {\hsp[-2][0, 0.00]} &  0.012839 &  {\hsp[-2][0, 0.07]} &   &  0.000000 &  {\hsp[-2][0, 0.01]} &  0.000000 &  {\hsp[-2][0, 0.00]} &  0.012839 &  {\hsp[-2][0, 0.07]} \\
MW  &  0.031855 		&  0.039365 &  {\hsp[-2][0, 0.16]} &  0.015509 &  {\hsp[-2][0, 0.07]} &   &  0.000000 &  {\hsp[-2][0, 0.02]} &  0.000000 &  {\hsp[-2][0, 0.01]} &  0.011947 &  {\hsp[-2][0, 0.07]} \\
EW  &  0.035415 		&  0.040444 &  {\hsp[-2][0, 0.13]} &  0.015663 &  {\hsp[-2][0, 0.07]} &   &  0.000000 &  {\hsp[-2][0, 0.03]} &  0.000000 &  {\hsp[-2][0, 0.01]} &  0.013230 &  {\hsp[-2][0, 0.07]} \\
QLR &  0.044251 		&  0.047740 &  {\hsp[-2][0, 0.16]} &  0.023180 &  {\hsp[-2][0, 0.09]} &   &  0.000000 &  {\hsp[-2][0, 0.04]} &  0.000000 &  {\hsp[-2][0, 0.03]} &  0.020805 &  {\hsp[-2][0, 0.08]} \\










% {\hsp[-2][0, 0.03]}
% {\hsp[-2][0, 0.08]}
% {\hsp[-2][0, 0.08]}
% {\hsp[-2][0, 0.09]}

==> table.input/Table_MUEb_CA.tex <==
$L$ &  {\hsp[2]---} &  0.037529 &  {\hsp[-2](0.9450{)}} &  0.048128 &  {\hsp[-2](0.8850{)}} &   &  0.038851 &  {\hsp[-2](0.9350{)}} &  0.037529 &  {\hsp[-2](0.9450{)}} &  0.048128 &  {\hsp[-2](0.8850{)}} \\
MW  &  0.833493 		&  0.824762 &  {\hsp[-2](0.4200{)}} &  0.182530 &  {\hsp[-2](0.9550{)}} &   &  0.221949 &  {\hsp[-2](0.9200{)}} &  0.214878 &  {\hsp[-2](0.9250{)}} &  0.278728 &  {\hsp[-2](0.8650{)}} \\
EW  &  0.801254 		&  0.761333 &  {\hsp[-2](0.2900{)}} &  0.101482 &  {\hsp[-2](0.9500{)}} &   &  0.126872 &  {\hsp[-2](0.9100{)}} &  0.122280 &  {\hsp[-2](0.9200{)}} &  0.161823 &  {\hsp[-2](0.8550{)}} \\
QLR &  8.513039 		&  8.272703 &  {\hsp[-2](0.0550{)}} &  1.514397 &  {\hsp[-2](0.8850{)}} &   &  1.842522 &  {\hsp[-2](0.8050{)}} &  1.793354 &  {\hsp[-2](0.8200{)}} &  2.040637 &  {\hsp[-2](0.7600{)}} \\



==> table.input/Table_MUEb_EA.tex <==
$L$ &  {\hsp[2]---} &  0.067682 &  {\hsp[-2](0.7650{)}} &  0.068424 &  {\hsp[-2](0.7600{)}} &   &  0.097108 &  {\hsp[-2](0.5950{)}} &  0.067682 &  {\hsp[-2](0.7650{)}} &  0.068424 &  {\hsp[-2](0.7600{)}} \\
MW  &  1.493978 		&  1.270378 &  {\hsp[-2](0.2500{)}} &  0.351069 &  {\hsp[-2](0.7900{)}} &   &  0.622436 &  {\hsp[-2](0.5450{)}} &  0.454903 &  {\hsp[-2](0.6850{)}} &  0.455205 &  {\hsp[-2](0.6850{)}} \\
EW  &  1.525650 		&  1.090316 &  {\hsp[-2](0.1750{)}} &  0.226251 &  {\hsp[-2](0.7500{)}} &   &  0.474062 &  {\hsp[-2](0.4550{)}} &  0.300121 &  {\hsp[-2](0.6400{)}} &  0.292027 &  {\hsp[-2](0.6500{)}} \\
QLR &  9.882686 		&  8.878605 &  {\hsp[-2](0.0450{)}} &  2.652280 &  {\hsp[-2](0.6150{)}} &   &  4.796794 &  {\hsp[-2](0.2650{)}} &  3.454149 &  {\hsp[-2](0.4500{)}} &  3.257853 &  {\hsp[-2](0.4900{)}} \\



==> table.input/Table_MUEb_UK.tex <==
$L$ &  {\hsp[2]---} &  0.080184 &  {\hsp[-2](0.6900{)}} &  0.081772 &  {\hsp[-2](0.6800{)}} &   &  0.079305 &  {\hsp[-2](0.6900{)}} &  0.080184 &  {\hsp[-2](0.6900{)}} &  0.081772 &  {\hsp[-2](0.6800{)}} \\
MW  &  1.295177 		&  1.319085 &  {\hsp[-2](0.2400{)}} &  0.309463 &  {\hsp[-2](0.8300{)}} &   &  0.540538 &  {\hsp[-2](0.6100{)}} &  0.546107 &  {\hsp[-2](0.6050{)}} &  0.555764 &  {\hsp[-2](0.6000{)}} \\
EW  &  0.984618 		&  1.021807 &  {\hsp[-2](0.1900{)}} &  0.210029 &  {\hsp[-2](0.7750{)}} &   &  0.392172 &  {\hsp[-2](0.5350{)}} &  0.397701 &  {\hsp[-2](0.5300{)}} &  0.409986 &  {\hsp[-2](0.5150{)}} \\
QLR &  5.993069 		&  6.261263 &  {\hsp[-2](0.1400{)}} &  3.541260 &  {\hsp[-2](0.4350{)}} &   &  4.408113 &  {\hsp[-2](0.3050{)}} &  4.476559 &  {\hsp[-2](0.2950{)}} &  4.619930 &  {\hsp[-2](0.2800{)}} \\



==> table.input/Table_MUEb_US.tex <==
$L$ &  {\hsp[2]---} &  0.037097 &  {\hsp[-2](0.9450{)}} &  0.170077 &  {\hsp[-2](0.3350{)}} &   &  0.049609 &  {\hsp[-2](0.8750{)}} &  0.037097 &  {\hsp[-2](0.9450{)}} &  0.170077 &  {\hsp[-2](0.3350{)}} \\
MW  &  2.747739 	  &  3.850795 &  {\hsp[-2](0.0150{)}} &  1.159557 &  {\hsp[-2](0.2850{)}} &   &  0.326527 &  {\hsp[-2](0.8150{)}} &  0.251819 &  {\hsp[-2](0.8900{)}} &  0.977255 &  {\hsp[-2](0.3550{)}} \\
EW  &  2.553645 	  &  3.184074 &  {\hsp[-2](0.0100{)}} &  0.775920 &  {\hsp[-2](0.2800{)}} &   &  0.199023 &  {\hsp[-2](0.7900{)}} &  0.148746 &  {\hsp[-2](0.8750{)}} &  0.681178 &  {\hsp[-2](0.3250{)}} \\
QLR &  12.398151    & 13.725281 &  {\hsp[-2](0.0050{)}} &  6.156285 &  {\hsp[-2](0.1450{)}} &   &  2.759496 &  {\hsp[-2](0.5900{)}} &  2.185052 &  {\hsp[-2](0.7200{)}} &  5.613296 &  {\hsp[-2](0.1850{)}} \\



==> table.input/Table_S2a_CA.tex <==
$\hsp[3]a_{y,1}  $               &  1.51416741 &  1.50661160 &  1.50350142 &  1.50345436 \\
$\hsp[3]a_{y,2}  $               & -0.56685374 & -0.56099271 & -0.55721560 & -0.55726716 \\
$\hsp[3]a_{r}    $               & -0.06316858 & -0.06320757 & -0.06464245 & -0.06462353 \\
$\hsp[3]a_{0}    $               & -0.09530898 & -0.08051874 &  {\hsp[7]---} & -0.00194468 \\
$\hsp[3]a_{g}    $               &  0.37648328 &  0.35430683 &  {\hsp[7]---} &  {\hsp[7]---} \\
$\hsp[3]b_{\pi } $               &  0.49581071 &  0.49508618 &  0.49588056 &  0.49580141 \\
$\hsp[3]b_{y}    $               &  0.06028640 &  0.06298155 &  0.06225903 &  0.06251268 \\
$\hsp[3]\sigma _{\tilde{y}}$     &  0.39785436 &  0.40457205 &  0.40900867 &  0.40901255 \\
$\hsp[3]\sigma _{\pi }     $     &  1.38008373 &  1.37954979 &  1.38020487 &  1.38014281 \\
$\hsp[3]\sigma _{y^{\ast }}$     &  0.58052963 &  0.57458703 &  0.57205197 &  0.57203639 \\
$\hsp[3]\sigma _{g}$ {(implied)} &  (0.02978747{)} &  0.03253349 &  0.03365829 &  0.03370739 \\
$\hsp[3]\lambda_g  $ {(implied)} &  0.05131085 &  (0.05662065{)} &  (0.05883782{)} &  (0.05892525{)} \\



==> table.input/Table_S2a_EA.tex <==
$\hsp[3]a_{y,1}  $               &  1.67569238 &  1.65132235 &  1.64793379 &  1.64998942 \\
$\hsp[3]a_{y,2}  $               & -0.72521483 & -0.70073480 & -0.69810738 & -0.70021725 \\
$\hsp[3]a_{r}    $               & -0.03196558 & -0.03844292 & -0.03809636 & -0.03833377 \\
$\hsp[3]a_{0}    $               & -0.03713846 &  0.00001298 &  {\hsp[7]---} & -0.01615968 \\
$\hsp[3]a_{g}    $               &  0.18359716 &  0.12015634 &  {\hsp[7]---} &  {\hsp[7]---} \\
$\hsp[3]b_{\pi } $               &  0.67855387 &  0.68419026 &  0.68308911 &  0.68314565 \\
$\hsp[3]b_{y}    $               &  0.08063733 &  0.06764999 &  0.07237657 &  0.07013818 \\
$\hsp[3]\sigma _{\tilde{y}}$     &  0.29347242 &  0.31175812 &  0.31237407 &  0.31136118 \\
$\hsp[3]\sigma _{\pi }     $     &  0.97845481 &  0.98011309 &  0.97997051 &  0.97984474 \\
$\hsp[3]\sigma _{y^{\ast }}$     &  0.39318254 &  0.37062132 &  0.37015853 &  0.37076399 \\
$\hsp[3]\sigma _{g}$ {(implied)} & (0.01391225{}) &  0.02588260 &  0.02561295 &  0.02574558 \\
$\hsp[3]\lambda_g  $ {(implied)} &  0.03538370 & (0.06983570{}) & (0.06919454{}) & (0.06943928{}) \\


==> table.input/Table_S2a_UK.tex <==
$\hsp[3]a_{y,1}  $               &  1.85797662 &  1.85829707 &  1.85897395 &  1.85774435 \\
$\hsp[3]a_{y,2}  $               & -0.94297465 & -0.94345380 & -0.94429692 & -0.94274276 \\
$\hsp[3]a_{r}    $               & -0.00844679 & -0.00834790 & -0.00827675 & -0.00845896 \\
$\hsp[3]a_{0}    $               & -0.01702065 & -0.01738443 &  {\hsp[7]---} & -0.00472266 \\
$\hsp[3]a_{g}    $               &  0.05467354 &  0.05512076 &  {\hsp[7]---} &  {\hsp[7]---} \\
$\hsp[3]b_{\pi } $               &  0.59294069 &  0.59286359 &  0.59284731 &  0.59314094 \\
$\hsp[3]b_{y}    $               &  0.54294214 &  0.54451716 &  0.54717393 &  0.54046566 \\
$\hsp[3]\sigma _{\tilde{y}}$     &  0.10528595 &  0.10478282 &  0.10380406 &  0.10578418 \\
$\hsp[3]\sigma _{\pi }     $     &  2.64036422 &  2.64027249 &  2.64024940 &  2.64066309 \\
$\hsp[3]\sigma _{y^{\ast }}$     &  0.85639356 &  0.85750606 &  0.85786256 &  0.85708628 \\
$\hsp[3]\sigma _{g}$ {(implied)} & (0.02033305{)} &  0.01808682 &  0.01819781 &  0.01831081 \\
$\hsp[3]\lambda_g  $ {(implied)} &  0.02374264 &  (0.02109236{)} & (0.02121297{)} &  (0.02136402{)} \\



==> table.input/Table_S2a_US.tex <==
$\hsp[3]a_{y,1}  $               &  1.51438668 &  1.47605057 &  1.51817784 &  1.51186045 \\
$\hsp[3]a_{y,2}  $               & -0.57128595 & -0.53488829 & -0.57824253 & -0.57230827 \\
$\hsp[3]a_{r}    $               & -0.07346174 & -0.08402097 & -0.06825241 & -0.07164411 \\
$\hsp[3]a_{0}    $               & -0.38877981 & -0.39331138 &  {\hsp[7]---} & -0.04299913 \\
$\hsp[3]a_{g}    $               &  0.75724701 &  0.79592000 &  {\hsp[7]---} &  {\hsp[7]---} \\
$\hsp[3]b_{\pi } $               &  0.66838723 &  0.67179221 &  0.67465713 &  0.67160611 \\
$\hsp[3]b_{y}    $               &  0.07934934 &  0.07552146 &  0.07710993 &  0.08112417 \\
$\hsp[3]\sigma _{\tilde{y}}$     &  0.33550730 &  0.32902106 &  0.34846403 &  0.34552731 \\
$\hsp[3]\sigma _{\pi }     $     &  0.78523542 &  0.78643123 &  0.78785015 &  0.78662062 \\
$\hsp[3]\sigma _{y^{\ast }}$     &  0.56797409 &  0.56163865 &  0.56051398 &  0.56064660 \\
$\hsp[3]\sigma _{g}$ {(implied)} & (0.03042073{)}&  0.04275448 &  0.04348429 &  0.04606357 \\
$\hsp[3]\lambda_g  $ {(implied)} & 0.05356007  &  (0.07612453{)} & (0.07757932{)} &  (0.08216150{)} \\


==> table.input/Table_S2b_CA.tex <==
{Log-likelihood} & -679.90156186 & -679.87545118 & -679.94373632 & -679.94347472 \\



==> table.input/Table_S2b_EA.tex <==
{Log-likelihood} & -422.30013304 & -421.13354157 & -421.17804744 & -421.13660601 \\



==> table.input/Table_S2b_UK.tex <==
{Log-likelihood} & -877.75517435 & -877.74815473 & -877.76354886 & -877.74887189 \\



==> table.input/Table_S2b_US.tex <==
{Log-likelihood} & -534.57461094 & -534.37024579 & -535.95791031 & -535.57316476 \\



==> table.input/Table_S3a_CA.tex <==
$\hsp[3]a_{y,1}  $                &  1.51607878 &  1.50339829 &  1.50339829 \\
$\hsp[3]a_{y,2}  $                & -0.56686382 & -0.55701526 & -0.55701526 \\
$\hsp[3]a_{r}    $                & -0.06620560 & -0.06454512 & -0.06454513 \\
$\hsp[3]b_{\pi } $                &  0.49906078 &  0.49635743 &  0.49635744 \\
$\hsp[3]b_{y}    $                &  0.05221334 &  0.06093603 &  0.06093604 \\
$\hsp[3]\sigma _{\tilde{y}}$      &  0.39354845 &  0.40917902 &  0.40917901 \\
$\hsp[3]\sigma _{\pi }     $      &  1.38253182 &  1.38055866 &  1.38055867 \\
$\hsp[3]\sigma _{y^{\ast }}$      &  0.58417740 &  0.57200959 &  0.57200960 \\
$\hsp[3]\sigma _{g}$ {(implied)}  &  (0.02997464{)} &  0.03366297 &  0.03366297 \\
$\hsp[3]\sigma _{z}$ {(implied)}  &  (0.09697384{)} &  (0.00000000{)} &  0.00000001 \\
$\hsp[3]\lambda_g  $ {(implied)}  &  0.05131085 		&  (0.05885035{)} &  (0.05885035{)} \\
$\hsp[3]\lambda_z  $ {(implied)}  &  0.01631365 		&  0.00000000 &  (0.00000000{)} \\



==> table.input/Table_S3a_EA.tex <==
$\hsp[3]a_{y,1}  $                &  1.67182426 &  1.64822319 &  1.64822319 \\
$\hsp[3]a_{y,2}  $                & -0.72246599 & -0.69843909 & -0.69843909 \\
$\hsp[3]a_{r}    $                & -0.03630451 & -0.03767476 & -0.03767476 \\
$\hsp[3]b_{\pi } $                &  0.68844980 &  0.68370935 &  0.68370935 \\
$\hsp[3]b_{y}    $                &  0.06512193 &  0.07134921 &  0.07134919 \\
$\hsp[3]\sigma _{\tilde{y}}$      &  0.28941500 &  0.31252152 &  0.31252152 \\
$\hsp[3]\sigma _{\pi }     $      &  0.98154863 &  0.98015826 &  0.98015826 \\
$\hsp[3]\sigma _{y^{\ast }}$      &  0.39412651 &  0.37012107 &  0.37012107 \\
$\hsp[3]\sigma _{g}$ {(implied)}  & (0.01394565{)} &  0.02559315 	&  0.02559315 \\
$\hsp[3]\sigma _{z}$ {(implied)}  & (0.26203109{)} & (0.00000000{)} 	&  0.00000003 \\
$\hsp[3]\lambda_g  $ {(implied)}  &  0.03538370 	 & (0.06914804{)}  	&  (0.06914804{)} \\
$\hsp[3]\lambda_z  $ {(implied)}  &  0.03286945 	 &  0.00000000  		&  (0.00000000{)} \\



==> table.input/Table_S3a_UK.tex <==
$\hsp[3]a_{y,1}  $                &  1.86610365 &  1.85954365 &  1.85954366 \\
$\hsp[3]a_{y,2}  $                & -0.95436885 & -0.94521873 & -0.94521874 \\
$\hsp[3]a_{r}    $                & -0.00710513 & -0.00806411 & -0.00806411 \\
$\hsp[3]b_{\pi } $                &  0.59266882 &  0.59271992 &  0.59271992 \\
$\hsp[3]b_{y}    $                &  0.56863226 &  0.55055550 &  0.55055551 \\
$\hsp[3]\sigma _{\tilde{y}}$      &  0.09058094 &  0.10269455 &  0.10269454 \\
$\hsp[3]\sigma _{\pi }     $      &  2.64007048 &  2.64009311 &  2.64009311 \\
$\hsp[3]\sigma _{y^{\ast }}$      &  0.86136819 &  0.85828959 &  0.85828959 \\
$\hsp[3]\sigma _{g}$ {(implied)}  &  (0.02045116{)} &  0.01817073 &  0.01817073 \\
$\hsp[3]\sigma _{z}$ {(implied)}  &  (0.24614394{)} &  (0.00000000{)} &  0.00000007 \\
$\hsp[3]\lambda_g  $ {(implied)}  &  0.02374264 		&  (0.02117087{)} &  (0.02117087{)} \\
$\hsp[3]\lambda_z  $ {(implied)}  &  0.01930743 		&  0.00000000 &  (0.00000001{)} \\



==> table.input/Table_S3a_US.tex <==
$\hsp[3]a_{y,1}  $                &  1.53991114 		&  1.51796245 	  &  1.51804519 \\
$\hsp[3]a_{y,2}  $                & -0.59855575 		& -0.57839056 	  & -0.57846939 \\
$\hsp[3]a_{r}    $                & -0.06786964 		& -0.06955268 	  & -0.06941225 \\
$\hsp[3]b_{\pi } $                &  0.67083803 		&  0.67182760 	  &  0.67187993 \\
$\hsp[3]b_{y}    $                &  0.07859265 		&  0.07984256 	  &  0.07985050 \\
$\hsp[3]\sigma _{\tilde{y}}$      &  0.33378693 		&  0.34501847 	  &  0.34535766 \\
$\hsp[3]\sigma _{\pi }     $      &  0.78620285 		&  0.78669831 	  &  0.78672365 \\
$\hsp[3]\sigma _{y^{\ast }}$      &  0.57390968 		&  0.56180867 	  &  0.56167781 \\
$\hsp[3]\sigma _{g}$ {(implied)}  & (0.03073865{)} 	&  0.04395352 	  &  0.04391602 \\
$\hsp[3]\sigma _{z}$ {(implied)}  & (0.17417263{)} 	& (0.06562814{)}  &  0.06237003 \\
$\hsp[3]\lambda_g  $ {(implied)}  &  0.05356007 		& (0.07823575{)}  & (0.07818721{)} \\
$\hsp[3]\lambda_z  $ {(implied)}  &  0.03541491 		&  0.01323005 	  & (0.01253554{)} \\



==> table.input/Table_S3b_CA.tex <==
{Log-likelihood} & -680.25212417 & -680.00345718 & -680.00345718 \\



==> table.input/Table_S3b_EA.tex <==
{Log-likelihood} & -422.87276090 & -421.23654260 & -421.23654260 \\



==> table.input/Table_S3b_UK.tex <==
{Log-likelihood} & -877.97896968 & -877.77522874 & -877.77522874 \\



==> table.input/Table_S3b_US.tex <==
{Log-likelihood} & -536.48377160 & -535.97760443 & -535.97718006 \\



==> table.input/_table1_notes.tex <==
%TCIDATA{Version=5.50.0.2953}
%TCIDATA{LaTeXparent=0,0,hlw.1a.tex}
This table reports parameter estimates of the various Stage 2 models. The
first column (`HLW.R-File') lists the estimates obtained from %
\cites{holston.etal:2017} R-Files, where $\lambda _{g}$ is fixed at the first
stage estimate and $\sigma _{g}$ is implied from the Stage 1 signal-to-noise
ratio $\lambda _{g}=\sigma _{g}/\sigma _{y^{\ast }}$. The second column
(`HLW($\hat{\sigma}_{g}^{\mathsf{MLE}}$)') shows estimates of the same model,
but with $\sigma _{g}$ computed by MLE together with the other parameters of
HLW's (misspecified) Stage 2 model shown in the right column block of
\ref{eq:S2}. The third column (`Correct') provides estimates of the correct
Stage 2 model defined in the left column block of \ref{eq:S2}, where $\sigma
_{g}$ is again estimated directly by MLE. The last column (`Correct +
$a_{0}$') shows estimates of the correct Stage 2 model when an additional
intercept term is added to the specification. Values in round brackets give
the implied values of $\sigma _{g}$ or $ \lambda _{g}$ from the $\lambda
_{g}=\sigma _{g}/\sigma _{y^{\ast }}$ relation when either $\lambda _{g}$ or
$\sigma _{g}$ are estimated.


==> table.input/_table2_notes.tex <==
%TCIDATA{Version=5.50.0.2953}
%TCIDATA{LaTeXparent=0,0,hlw.1a.tex}
This table reports the Stage 2 MUEs of $\lambda_{z}$ and corresponding
structural break statistics computed from the correct Stage 2 model and HLW's
(misspecified) Stage 2 model defined in the left and right columns of
\ref{eq:S2}, respectively. The table is split into a left and right block
corresponding to the two different implementations of the structural break
regressions for each of the Stage 2 models defined in equations \ref{d_hlw}
to \ref{d_true0}. The left block shows HLW's implementation of the structural
break regressions. The right block shows SW's implementation. The table is
further split into a top and bottom half. The top half shows the MUEs of
$\lambda_z$. The bottom half lists the corresponding structural break test
statistics. The results under (`HLW.R-File') report $\lambda _{z}$ estimates
obtained from \cites{holston.etal:2017} R-Files for HLW's (misspecified)
Stage 2 model. The (`HLW($\hat{\sigma}_{g}^{\mathsf{MLE}}$)') column lists
estimates of the same model but with $\sigma _{g}$ estimated directly by MLE\
rather than from the first Stage $\lambda _{g}$. Results under the heading
(`Correct') are for the correct Stage 2 model, where $\sigma _{g}$ is again
estimated directly by MLE. The table lists
results for all four structural break tests, namely, \cites{nyblom:1989} $L$%
, MW, EW and QLR tests. Values in square brackets in the top part of the
table are $90\%$ lower and upper confidence intervals (CIs). Values in
parenthesis in the bottom part are $p-$values corresponding to SW's
structural break tests. Both, the CIs as well as the $p-$values, were
obtained from \cites{stock.watson:1998} GAUSS\ files.




%test implementations, which are denoted by `Time varying $\boldsymbol{\phi
%}$' and `Constant $\boldsymbol{\phi }$', respectively.


==> table.input/_table3_notes.tex <==
%TCIDATA{Version=5.50.0.2953}
%TCIDATA{LaTeXparent=0,0,hlw.1a.tex}
This table reports the Stage 3 estimates. The first column (`HLW.R-File')
gives the estimates from \cites{holston.etal:2017} R-Files. The second column
(`MLE$(\sigma _{g}|\hat{\lambda}_{z}^{\mathrm{Correct}})$') shows estimates
of $\lambda _{z}$ from the correct Stage 2 model and SW's implementation of
the structural break regressions in \ref{d_true0} (based on the EW structural
break test), where $\sigma _{g}$ is again estimated by MLE. The last column
(`MLE$(\sigma _{g},\sigma _{z})$') reports estimates where all parameters,
including $(\sigma _{g},\sigma _{z})$, are computed directly by MLE. Values
in round brackets give the implied $(\sigma _{g},\sigma _{z})$ or $(\lambda
_{g},\lambda _{z})$ values constructed from the signal-to-noise ratios
$\lambda _{g}=\sigma _{g}/\sigma _{y^{\ast }}$ and $\lambda _{z}=a_{r}\sigma
_{z}/\sigma _{\tilde{y}}$.


%of $\lambda _{z}$ ($\hat{\lambda}_{z}^{\mathrm{Correct}}$) ($\hat{\lambda}_{z}^{\mathrm{Correct}}$)

